Automatic Raman Measurements in a High-Throughput Bioprocess Development Lab

This study presents a collection of physical devices and software services that fully automate Raman spectra measurements for liquid samples within a robotic facility. This method is applicable to various fields, with demonstrated efficacy in biotechnology, where Raman spectroscopy monitors substrates, metabolites, and product-related concentrations. Our system specifically measures 50 $\micro L$ samples using a liquid handling robot capable of taking 8 samples simultaneously. We record multiple Raman spectra for 10s each. Furthermore, our system takes around 20s for sample handling, cleaning, and preparation of the next measurement. All spectra and metadata are stored in a database, and we use a machine learning model to estimate concentrations from the spectra. This automated approach enables gathering spectra for various applications under uniform conditions in high-throughput fermentation processes, calibration procedures, and offline evaluations. This allows data to be combined to train sophisticated machine learning models with improved generalization. Consequently, we can develop accurate models more quickly for new applications by reusing data from prior applications, thereby reducing the need for extensive calibration data.

==> Matrial_liste.tex <==
\begin{table}[!ht]
    \centering
    \begin{adjustbox}{angle=90}
    \begin{tabular}{|l|l|}
    \hline
        10 & Nut, flangeless, PPS, 1/16'' OD, Headless, 1pc/PAK \\ \hline
        2 & Flangeless Ferrule Tefzel (ETFE), 1/4-28 Flat-Bottom, for 1/16'' OD blue, 10pc/PAK \\ \hline
        1 & Tubing, PTFE, 1/16 x 1.0 mm ID, 25 m/PAK \\ \hline
        1 & Flangeless fitting PEEK 1/16in, 10 pc/PAK \\ \hline
        1 & Flangeless Ferrule, for 2.0mm OD, 10 pc/PAK \\ \hline
        2 & NS1D48042812 - CPC Stecker 1/4-28 UNF Innengewinde (Flat Bottom Port), mit Absperrventil, EPDM-Dicht \\ \hline
        2 & NS1D19042812 - CPC Kupplung 1/4-28 UNF Innengewinde (Flat Bottom Port), mit Absperrventil, EPDM-Dich \\ \hline
        1 & PMCD4204 - CPC Kupplung Stecker 6,4 mm Schlauchanschluss, Plattenmontage, mit Absperrventil, Buna-N \\ \hline
        1 & PMCD1704 - Kupplung 6,4 mm Schlauchanschluss, mit Absperrventil, Buna-N Dichtung \\ \hline
        1 & Idex – Hersteller Nr. P-387X – Artikelnummer GZ-02022-09 \\ \hline
        1 & Idex – Hersteller Nr. P-352X – Artikelnummer GZ-02021-95 \\ \hline
        1 & Flangeless Ferrule Ferrule, Tefzel (ETFE), for 1/16'' OD, 10 pc/PAK \\ \hline
        10 & Nut, flangeless, PPS, 1/16'' OD, Headless, 1pc/PAK \\ \hline
        2 & Huenersdorf™ Weithals-Kanister aus HDPE mit UV-Schutz \\ \hline
        1 & Tefzel (ETFE) Schlauch, natur, 1/16'' AD, 0,010'' ID, 15 m, 1 St/Pkg \\ \hline
        1 & Tefzel (ETFE) Schlauch, natur, 1/16'' AD, 0,020'' ID, 15 m, 1 St/Pkg \\ \hline
        1 & Außenmutter, superflanschlos, PEEK, kurz, kopflos, M6 Flachboden, für 1/16'' AD, 10 St/Pkg \\ \hline
        1 & Ferrule, superflanschlos, PEEK, 1/4-28 Flachboden, 1/16'' AD, natur, 10 St/Pkg \\ \hline
        1 & Ferrule, superflanschlos, mit Edelstahlring, 1/4-28 Flachboden, für 1/16'' AD, natur, 10 St/Pkg \\ \hline
    \end{tabular}
    
\end{adjustbox}
\end{table}
